SkyScapes -- Fine-Grained Semantic Understanding of Aerial Scenes

Understanding the complex urban infrastructure with centimeter-level accuracy is essential for many applications from autonomous driving to mapping, infrastructure monitoring, and urban management. Aerial images provide valuable information over a large area instantaneously; nevertheless, no current dataset captures the complexity of aerial scenes at the level of granularity required by real-world applications. To address this, we introduce SkyScapes, an aerial image dataset with highly-accurate, fine-grained annotations for pixel-level semantic labeling. SkyScapes provides annotations for 31 semantic categories ranging from large structures, such as buildings, roads and vegetation, to fine details, such as 12 (sub-)categories of lane markings. We have defined two main tasks on this dataset: dense semantic segmentation and multi-class lane-marking prediction. We carry out extensive experiments to evaluate state-of-the-art segmentation methods on SkyScapes. Existing methods struggle to deal with the wide range of classes, object sizes, scales, and fine details present. We therefore propose a novel multi-task model, which incorporates semantic edge detection and is better tuned for feature extraction from a wide range of scales. This model achieves notable improvements over the baselines in region outlines and level of detail on both tasks.

==> sections/comments.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%COMMENTED TEXT FROM ABSTRACT AND INTRODUCTION%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Abstract}
%   Understanding of complex infrastructures with centimeter-level accuracy has been a long needed tool for a wide range of applications to create high resolution maps for autonomous driving, mapping, infrastructure monitoring, urban management.
   
%   While airborne images provide valuable information in short period of time over a large area and although aerial object detection has benefited enormously from large-scale datasets, especially in the context of deep learning, for semantic understanding, however, no current dataset  adequately  captures  the  complexity  of real-world aerial scenes. 
   
%   % sentence on aerial perspective being better for large-scale mapping than ground-view?
   
%   To address this, we introduce \skyscapes, a benchmark to train and test approaches for pixel-level semantic labeling using airborne images. \skyscapes is the first aerial dataset with highly accurate, fine-grained annotations to enable the development of such methods.
   
%     call it 31 (20+12-1) classes or mention the two setting separately
%   \skyscapes is comprised of a diverse set of classes with detailed annotations of 31 classes ranging from large structures, such as buildings, roads and vegetation, to very fine details, such as lane markings on roads.
%   % mention shortly benchmarks
%   We have derived two main benchmarks on dense object segmentation and multi-class lane-markings and three auxiliary benchmarks on multi-class/binary edge detection and the simplified version.
   
%   We carry out several experiment to evaluate state-of-the art methods for pixel-wise semantic segmentation on the \skyscapes dataset.
   
%     Can we make this claim about our baseline models? #Majid: yes, based o the results, I think we can.
%   Our results show that it is very challenging for existing methods to deal with the range of classes, sizes, scales and fine details in the dataset.
%   Particularly edges, occluded/shadowed areas, and merged regions are a common type of error.
   
%   We thus further propose a novel multi-task model for semantic segmentation enabling feature extraction from the large range of sizes which incorporates semantic edge detection and achieves a notable improvement in region outlines and level of detail on both benchmarks.
%     Is this claim supported by the numbers? #Majid: yes, it will supported by the numbers.
%   \TODO{review, adapt claims}
%   The \skyscapes dataset will be publicly available at \url{[redacted-for-review]}.%.\url{https://www.dlr.de/eoc/en}.
   
% \section{Introduction}
% \sampledifferentAnnotations
% Automated methods for creating models or maps of today's wide-spread infrastructures with \gls{cml} accuracy are of great aid in handling the growing complexity of infrastructure management, optimization, analysis, or maintenance.

% A popular example for this is the application of \gls{HD} maps of road infrastructure to aid in autonomous driving tasks.
% Nowadays an automated analysis of public transportation networks is essential for the generation of accurate road maps and lane based models. A broad range of current systems, \eg navigation systems, assisted driving, and \gls{AV}, rely on such information.
% Arne: why 'future'; mention these applications bevore AV, since AV is our main focus below and this in between sort of breaks the flow
% Future applications, like continuous infrastructure monitoring, urban management, city planning, and general mapping, also require high precision maps at \gls{cml} accuracy.
% At present \gls{AV} are a research focus in computer vision and remote sensing.
% In order to achieve autonomy in \glspl{AV}, one key factor is to localize the vehicle precisely.
% Arne: @majid: undefined command here: \goal
% Very accurate maps containing the location of infrastructures, such as streets, sidewalks, traffic lights and even lane markings, are a necessity for reaching the goal of fully autonomous driving.
% \Gls{ADAS} comprising features like vehicle navigation and lane departure warning requires not only the road model information, but also the precise road lane marking data, \eg the lane marking types and their locations.

% This ranges from the use of a general road network for navigation purposes to more advanced automation tasks, which rely on detailed road network models, including the locations of lane boundaries, bike lanes, sidewalks, pedestrian crossings and other road marks \cite{poggenhans2018lanelet2,seif2016autonomous,mattyus2016hd,zheng2018high}.
% can we emphasize more clearly which concrete autonomous driving tasks require such detailed differentiation between lane markings? /majid: we will emphasize this when explaining the dataset esp. for the lane-markings. I added only one line about this for the related datasets.
% Arne: Reworked+shortened motivation paragraph

% At present the data collection for generating \gls{HD} maps is mainly carried out by so called mobile mapping systems, which comprise in most cases of a vehicle equipped with a broad range of sensors (\eg Radar, LiDAR, cameras) and followed by automated analysis of these ground-based sensors
% ~\cite{guo2016low,gwon2017generation,carneiro2018mapping,lamon2006mapping}.
% This task is complicated by the challenge of fusing the recorded information into a consistent map, as well as frequent occlusions of relevant details due to the low sensor angle. Also they come with other drawbacks, for instance the ground based systems can cover only a small part of the map due to the sensor line-of-sight. Sensor drift and \gls{GPS}-shadows in urban canyons lower the spatial accuracy, traffic flow leads to partial occlusions in the recorded data.
% The advantage of aerial imagery
% An aerial perspective can alleviate many of these problems and simultaneously allow for processing of much larger areas at once in a very short period of time with \gls{cml} geo-referenced data acquisition. Therefore, we could address this issue by remote sensing imagery which is intrinsically motivated by the need for large areas in short time at a monetary competitive level. More and more airborne and space-borne sensors recording data in the very-high resolution, \eg \gls{gls:GSD} less than \SI{50}{\cm} domain are in operational mode.
% The public sector often offers its data under a free-and-open policy, \eg aerial imagery of \gls{USGS} in urban regions has \gls{gls:GSD} less than \SI{30}{\cm}. Lower \gls{gls:GSD} up to even \SI{1}{\cm} can be achieved using airborne and \gls{UAV} imagery, but with smaller coverage.
% the shortcomings of current aerial datasets - postdam, torontocity, spacenet, 
% However, current aerial datasets are limited in the level of detail of their annotations and  provide segmentation information either for entire roads such as Postdam\cite{potsdam}, SpaceNet \cite{van2018spacenet}, DeepGlobe\cite{demir2018deepglobe}, INRIA\cite{maggiori2017dataset} or DataFusion\cite{debes2014hyperspectral} by fusing multi-spectral data including RGB data with LiDAR data or at most for road center-lines like TorontoCity\cite{wang2016torontocity}. For instance, these datasets lack the details of lane-markings with different classes which is of great importance for a autonomous vehicle to localize itself. Moreover, one could notice for instance entrance/exit regions, sidewalks, and bike-ways are also missing in current most recent datasets. 
% Arne: this addition seems arbitrary (of course there are datasets for different tasks)
% Other aerial and satellite datasets focus on object detection\cite{xia2018dota,majid2019vehicles}. \majid{shall we add more datasets? from my points these are the most important ones.}
% todo rephrase
% Regarding the lane-markings, the knowledge about the placement and appearance of lane markings is a prerequisite for the creation of maps with high precision, necessary for autonomous driving as they are one of the important components of such maps. Lane markings convey the rules of roads to drivers. While these rules are learned by humans, an autonomous driving vehicle should be taught to learn them to localize itself.

% Fisher et al.\cite{fischer2018towards} proposed method to detect lane-marking after road segmentation which is until recently the only way of lane-marking detection with limitation to 3rd-party sources such as OpenStreetMap and GoogleMap.  Mattyus et al.~\cite{mattyus2017deeproadmapper} proposed a method to alleviate this, but still focused on road segmentation based on Markov Random Fields and a combined parsing of both ground and aerial images to generate detailed maps. Azimi et al.~\cite{azimi2018aerial} however tried for the first time to tackle lane-marking localization for \gls{HD}mapping directly independent of any 3rd-party sources and regardless of the location of lane-marking while achieving very good results, but still limited to binary lane-marking. In this work, we have tried to bring it to the next and practical level by tackling multi-class lane-marking segmentation and still being free of 3rd-party data. 

% In this work, we provide a new aerial dataset, called SkyScapes, which closes this gap by providing detailed annotations of urban scenes for established classes, such as buildings, vegetation, divided into grass and trees, 
% roads, and parking-places, with paved and non-paved differentiation
% as well as much more 
% fine-grained classes, such as various types of lane markings, pedestrian crossings, bikeways, sidewalks, 
% vehicle entrance/exit zones, danger areas, which are the intersection of bikeways and roads, and even more. ~\cref{fig:differentannotation} shows different annotation types offered by \skyscapes including different lane-marking classes (also see~\cref{fig:signs}).
   
% \section{Semantic benchmarks}
% \subsection{State-of-the-art in Semantic Segmentation}

% We have two main benchmarks, SkyScapes-Dense and SkyScapes-Lane as well as three auxiliary benchmarks; SkyScapes-Dense-Merged, SkyScapes-Edge-Binary, and SkyScapes-Edge-Multi benchmarks using the method achieving the best performance on the main benchmarks.

% \TODO{qualitative analysis, what are typical error cases}
% % We have carried out an extensive benchmark on SkyScapes-Dense using different deep learning-based method starting with FCN~\cite{long2015fully} to the very recent ones such as DenseASPP~\cite{yang2018denseaspp} and BiSeNet~\cite{yu2018bisenet} due to their proven superior performance over traditional methods in the last few years.
% By evaluation of the results provided in ~\ref{tab:bchmkSkyscapesAllcls} and ~\ref{tab:bchmkSkyscapesEachcls}, we noticed almost all of the methods even the most recent ones have major struggle in achieving high performance on \skyscapes. This is due to the complexity of this task when it comes to aerial scenes which is more challenging compared to ground imagery because of the reasons mentioned in \ref{sec:intro}. By further investigation of the results, we noticed the majority of the errors occur in the boundary of different classes in which the methods are struggling to detect the border among different object classes in SkyScapes-Dense benchmark.
% \TODO{describe results, what are main observed differences from this eval setup compared to main classes, i.e. are there models which are very good on main classes but weak on lane types, etc.}
% Regarding SkyScapes-Lane benchmark provided in ~\ref{tab:bchmkSkyscapesMultiLaneAllcls} and ~\ref{tab:bchmkSkyscapesMultiLaneEachcls}, we observed a general consistency between the performance of the methods in Dense benchmark and Multi-class lane-marking one \ie the best performing methods in SkyScapes-Dense perform roughly as good in SkyScapes-Lane benchmark. It should be noted that SkyScapes-Lane is very challenging as it is so the best of our knowledge tackles the tiniest multi-class pixel-wise segmentation task ever created \eg \SI{3x3}{\px} lane-marking which we believe it would help the community to develop future methods for segmentation of very tiny objects.
% \TODO{qualitative analysis, what are typical error cases}
% By investigating the qualitative and quantitative results of the best performing benchmark, we noticed the considerable portion of the errors comes from confusion of lane-marking with the background \ie the method has serious struggle to detect lane-markings. 
% \TODO{conclusions regarding weaknesses of existing methods and motivation for own method}
% Therefore, by evaluating the methods on both benchmark we reached to the conclusion that in dense segmentation scenario and multi-class lane-marking one, we should focus on boundaries of neighboring objects and binary lane-marking localization to improve the performance of the current methods. 


==> sections/relwork.tex <==
%%%%%%%%% BODY TEXT
\section{Related works}
\label{sec:relwork}

\noindent\textbf{Semantic segmentation \& HD mapping}
\TODO{writing about other algorithms on semantic segmentation}
\TODO{talking about other works in remote sensing to tackle HD mapping}


%\TODO{Talk about other works for autonomous driving, cityscapes, kitti, mapillary, lane datasets}
%\TODO{writing about postdam dataset and similar datasets}
%\noindent\textbf{Datasets} % there is only one subsection. I think we should comment this.
Many large datasets exist that provide annotations for semantic segmentation from a ground vehicle's perspective \cite{scharwachter2013efficient,geiger2013vision,cordts2016cityscapes,neuhold2017mapillary,yu2018bdd100k,roberts2018dataset,pan2018SCNN}.
In most cases, the annotations of these datasets focus strongly vehicles, persons, road bounds, and traffic signs.
Lane marking types are not considered although some datasets provide lane boundary annotations \cite{yu2018bdd100k,roberts2018dataset,pan2018SCNN}.
The field-of-view in these datasets is strongly limited by vehicles and buildings.
Thus, the resulting scene segmentation can not easily be integrated into an \gls{HD} map and mapping of large urban areas in this way requires a lot of time and resources.
Moreover, the oblique view of in-situ cameras mounted on mapping vehicles makes it hard to have nadir view on objects to acquire absolute geo-coordinates. Even some works have tried to convert in-situ images to birdview ones to have a better understanding of surrounding object visually and locally\majid{I could not find the paper in ECCV18 on this}. This becomes even more challenging by occluding vehicles, pedestrians and other dynamic objects.

Fisher et al.\cite{fischer2018towards} proposed method to detect lane-marking after road segmentation which is until recently the only way of lane-marking detection with limitation to 3rd-party sources such as OpenStreetMap and GoogleMap.  Mattyus et al.~\cite{mattyus2017deeproadmapper} proposed a method to alleviate this, but still focused on road segmentation based on Markov Random Fields and a combined parsing of both ground and aerial images to generate detailed maps. Azimi et al.~\cite{azimi2018aerial} however tried for the first time to tackle lane-marking localization for \gls{HD}mapping directly independent of any 3rd-party sources and regardless of the location of lane-marking while achieving very good results, but still limited to binary lane-marking. In this work, we have tried to bring it to the next and practical level by tackling multi-class lane-marking segmentation and still being free of 3rd-party data. 
%Note: for now, I've excluded patch-based land-cover classification datasets (e.g. UCM, SpaceNet, AID, fMoW, etc.)
%Note: eo-learn land-cover dataset looks interesting but has no real reference: https://medium.com/sentinel-hub/land-cover-classification-with-eo-learn-part-1-2471e8098195
% vehicle instance segmentation: https://arxiv.org/pdf/1805.10485.pdf  
%majid: I think for now we can ignore the datasets only on one specific class such as vehicles, building and focus on the datasets which have more than one class. 
%shall we merge the related works part to introduction as the following part has partially been mentioned in introduction section.
Several datasets also focus on the task of semantic segmentation from an aerial perspective \cite{maggiori2017dataset,demir2018deepglobe,van2018spacenet,potsdam,wang2016torontocity,lyu2018uavid,semanticdrone}.
However, the annotations of these datasets are often limited to specific tasks.
The INRIA Aerial Image Labeling dataset \cite{maggiori2017dataset} focuses on the binary task of building footprint segmentation.
Similarly, the SpaceNet dataset \cite{van2018spacenet} provides annotations for either building footprints or road segmentation.
The DeepGlobe challenge dataset \cite{demir2018deepglobe} supports three tasks: road extraction, building detection, and coarse land cover classification.
The TorontoCity dataset \cite{wang2016torontocity} includes annotations for 10 classes in aerial images, allowing for specialized tasks, such as building segmentation, zoning segmentation, and road center-line and boundary estimation. However, the annotations are taken from maps, which can result in inaccuracies due to registration errors or outdated information.
The UAVid dataset \cite{lyu2018uavid} consists of videos recorded by a \gls{UAV} at an oblique camera angle. The dataset supports the development of semantic video segmentation methods for 8 coarse classes.
The Semantic Drone dataset \cite{semanticdrone} provides overhead videos at very low altitude with 20 annotated classes focused on a residential neighborhood.
%maybe leave these out, because not (just) RGB imagery?
% if we would not have enough space, we can leave it out.
Multispectral sensor data is included in the ISPRS Vaihingen dataset \cite{potsdam}, which provides infrared imagery for segmentation of 6 classes, and the GRSS Data Fusion Contest dataset \cite{debes2014hyperspectral}, which provides hyperspectral and LiDAR data for 15 land cover classes, but still with very coarse and noticeable noisy annotations.
%
Closest to SkyScapes is the ISPRS Potsdam dataset of the ISPRS semantic labeling contest \cite{potsdam}.
This dataset is recorded from an overhead angle at sufficient height for \gls{HD} mapping purposes. However, only 6 coarse classes are included in the dataset.
%majid: we should also mention the images have been taken in the early morning resulting in somehow dark images with a lot of shadows while skyscape was taken at noon with higher quality images however higher GSD of 13cm rather than 4cm.
A more detailed comparison between the ISPRS Potsdam dataset and \skyscapes is carried out in Section \ref{sec:properties}.

To our knowledge, \skyscapes is the first dataset to uniquely combine fine-grained annotations of road infrastructure with an overhead view angle and coverage of large areas, thus directly enabling the development and evaluation of \gls{HD} mapping techniques for various applications such as autonomous driving mapping.

